EASY: Ensemble Augmented-Shot Y-shaped Learning: State-Of-The-Art Few-Shot Classification with Simple Ingredients

Few-shot learning aims at leveraging knowledge learned by one or more deep learning models, in order to obtain good classification performance on new problems, where only a few labeled samples per class are available. Recent years have seen a fair number of works in the field, introducing methods with numerous ingredients. A frequent problem, though, is the use of suboptimally trained models to extract knowledge, leading to interrogations on whether proposed approaches bring gains compared to using better initial models without the introduced ingredients. In this work, we propose a simple methodology, that reaches or even beats state of the art performance on multiple standardized benchmarks of the field, while adding almost no hyperparameters or parameters to those used for training the initial deep learning models on the generic dataset. This methodology offers a new baseline on which to propose (and fairly compare) new techniques or adapt existing ones.

==> tables/ablations_yuqing/transductive.tex <==
\begin{table}[!htbp]
    \caption{Ablation study of the steps of propsoed solution in \textbf{transductive} setting, for a fixed number of trainable parameters in the considered backbones. When using ensembles, we use 2$\times$ResNet12$\left(\frac{1}{\sqrt{2}}\right)$ instead of a single ResNet12.}
    \label{tab:ablation_trans}
    \centering
    \begin{tabular}{ccccc}
    \toprule
    Dataset & E & AS & 1-shot & 5-shot\\
    \midrule
    \multirow{4}*{MiniImageNet} 
    & & & $79.88 \pm 0.24$ & $86.93\pm 0.13$ \\
    & & \checkmark & $81.43 \pm 0.24$ & $88.06 \pm 0.12$\\
    & \checkmark & & $80.91 \pm 0.24$ & $87.72 \pm 0.12$\\
    & \checkmark & \checkmark & $\mathbf{82.18\pm 0.24}$ & $\mathbf{88.57\pm 0.12}$\\
    \midrule
    \multirow{4}*{CUB-FS} 
    & & & $86.63 \pm 0.23$ & $91.50\pm 0.11$ \\
    & & \checkmark & $89.26\pm 0.26$ & $92.80\pm 0.10$\\
    & \checkmark & & $88.23 \pm 0.23$& $92.18\pm 0.10$\\
    & \checkmark & \checkmark & $\mathbf{90.25\pm 0.19}$&$\mathbf{93.29\pm 0.10}$ \\
    \midrule
    \multirow{4}*{CIFAR-FS} 
    & & & $84.86 \pm 0.24$ & $89.06 \pm 0.15$\\
    & & \checkmark & $85.61\pm 0.24$ & $89.66\pm 0.15$\\
    & \checkmark & & $86.26 \pm 0.23$ & $89.65 \pm 0.15$ \\
    & \checkmark & \checkmark & $\mathbf{86.40\pm 0.23}$ & $\mathbf{89.95 \pm 0.15}$\\
    \midrule
    \multirow{4}*{FC-100} 
    & & & $53.93\pm 0.24$ & $65.62\pm 0.20$\\
    & & \checkmark & $54.10\pm 0.24$ & $65.70\pm 0.20$\\
    & \checkmark & & $55.04 \pm 0.24$ & $66.36\pm 0.20$\\
    & \checkmark & \checkmark & $\mathbf{54.68 \pm 0.25}$& $\mathbf{66.38\pm 0.20}$\\
    \midrule
    \multirow{4}*{TieredImageNet} 
    & & & $82.26 \pm 0.27$ & $87.97\pm 0.15$\\
    & & \checkmark & $82.66 \pm 0.27$ & $88.60 \pm 0.14$\\
    & \checkmark & & $82.75\pm 0.26$ & $88.32 \pm 0.15$ \\
    & \checkmark & \checkmark & $\mathbf{83.07 \pm 0.27}$ & $\mathbf{88.85\pm 0.15}$\\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/inductive/table_inductive_CIFARFS.tex <==
\begin{table*}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on CIFAR-FS in the inductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
         \midrule
         S2M2R \cite{mangla2020charting} &ResNet18 &11M & \checkmark & & $63.66\pm 0.17\%$ & $76.07 \pm 0.19\%$ \\ % S2M2R
         
          R2-D2 (+ens) \cite{liu2020task} &ResNet12 &12M & \checkmark & \checkmark & $76.51\pm 0.47\%$ & $87.63 \pm 0.34\%$ \\ % R2-D2 (+ens) (+val)
         invariance-equivariance\cite{rizve2021exploring} & ResNet12 & 12M & \checkmark& & $\mathbf{77.87\pm0.85\%}$ & $\mathbf{89.74 \pm 0.57\%}$\\ %equivariance invariance
          EASY (ours) & 2$\times$ResNet12($\frac{1}{\sqrt{2}}$) & 12M & \checkmark & \checkmark & $75.24 \pm 0.20\%$ & $88.38 \pm 0.14\%$\\
       \midrule
 
        S2M2R \cite{mangla2020charting} & WRN-28-10 & 36M & & &$74.81\pm0.19\%$ & $87.47\pm0.13\%$\\ %S2M2R
         EASY (ours) & 3$\times$ResNet12 & 36M & \checkmark & \checkmark & $\mathbf{76.20\pm 0.20\%}$ & $\mathbf{89.00 \pm 0.14\%}$\\
         
    \bottomrule
    \end{tabular}
    \label{tab:results_inductive_CIFARFS}
\end{table*}


 % xu2020attentional 75.4 ± 0.2 86.8 ± 0.2
 
 % tian2020rethinking 73.9 ± 0.8 86.9 ± 0.5

==> tables/inductive/table_inductive_CUBFS.tex <==
\begin{table*}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on CUB-FS in the inductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
         \midrule
        FEAT \cite{Ye2018} & ConvNet & 0.1M & & & $68.87 \pm 0.22\%$ & $82.90\pm0.10\%$\\ % FEAT %113K parameters for conv4
         LaplacianShot \cite{MasudZiko2020} &ResNet18 &11M & & & $\mathbf{80.96\quad\quad\quad\%}$ & $88.68\quad\quad\quad\%$ \\ % Protonet

         ProtoNet \cite{Snell2017} &ResNet18 &11M & & & $66.09\pm0.92\%$ & $82.50\pm 0.58\%$ \\ % Protonet
          DeepEMD v2 \cite{zhang2020deepemd} &ResNet12 &12M &  & \checkmark & $79.27\pm 0.29\%$ & $89.80\pm 0.51\%$ \\ % DeepEMD
          EASY (ours) & 4$\times$ResNet12($\frac{1}{2}$) & 12M & \checkmark & \checkmark & $77.97 \pm 0.20\%$  & $\mathbf{91.59 \pm 0.10\%}$\\
       \midrule
 
        S2M2R \cite{mangla2020charting} & WRN-28-10 & 36M & & &$\mathbf{80.68\pm0.81\%}$ & $90.85\pm0.44\%$\\ %S2M2R
         EASY (ours) & 3$\times$ResNet12 & 36M & \checkmark & \checkmark & $78.56 \pm 0.19\%$ & $\mathbf{91.93 \pm 0.10\%}$\\
         
    \bottomrule
    \end{tabular}
    \label{tab:results_inductive_CUBFS}
\end{table*}



==> tables/inductive/table_inductive_FC-100.tex <==
\begin{table*}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on FC-100 in the inductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
         \midrule
        DeepEMD v2\cite{zhang2020deepemd} & ResNet10 & 12M & & \checkmark&$46.60\pm0.26\%  $&$ 63.22 \pm 0.71\%$ \\ 
        TADAM\cite{Oreshkin} &ResNet12 & 12M & & & $40.10 \pm 0.40\%$ & $56.10\pm 0.40\%$ \\
        ProtoNet\cite{Snell2017} &ResNet12 & 12M & & & $41.54 \pm 0.76\%$ & $57.08\pm 0.76\%$ \\ %ProtoNet
        invariance-equivariance \cite{rizve2021exploring} & ResNet12 & 12M& \checkmark& & $47.76  \pm 0.77\%$ & $\mathbf{65.30 \pm 0.76 \%}$\\ %equivariance invariance
        R2-D2 (+ens) \cite{liu2020task} &ResNet12 & 12M & \checkmark &  \checkmark&  $44.75\pm 0.43\%$ & $59.94\pm0.41 \%$ \\ 
        EASY (ours) & 2$\times$ResNet12($\frac{1}{\sqrt{2}}$) & 12M & \checkmark & \checkmark & $\mathbf{47.78 \pm 0.20\%}$ & $65.24 \pm 0.19\%$\\
         
    \bottomrule
    \end{tabular}
    \label{tab:results_inductive_FC100}
\end{table*}

% 

==> tables/inductive/table_inductive_miniImageNet.tex <==
\begin{table*}[!ht]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on miniImageNet in the inductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
         \midrule
        SimpleShot \cite{wang2019simpleshot} & ResNet18 & 11M & & &$62.85\pm0.20\%$ & $80.02\pm0.14\%$\\ %SimpleShot
        Baseline++ \cite{Chen2019} & ResNet10 & 12M& & & $53.97\pm0.79\%$ & $75.90\pm0.61\%$ \\ %Baseline++
        TADAM\cite{Oreshkin} &ResNet12 & 12M & & & $58.50 \pm 0.30\%$ & $76.70\pm 0.30\%$ \\
        ProtoNet \cite{Snell2017} & ResNet12 & 12M & & &$60.37\pm0.83\%$ & $78.02\pm0.57\%$\\ %ProtoNet
        R2-D2 (+ens) (+val) \cite{liu2020task} & ResNet12 & 12M & \checkmark &  \checkmark& $65.95\pm0.45\%$ & $81.96\pm0.32\%$\\
        FEAT \cite{Ye2018} & ResNet12 & 12M & & & $66.78\quad \quad \quad\%$ & $82.05\quad  \quad \quad \%$\\ % FEAT
        CNL \cite{zhao2021looking} & ResNet12 & 12M & & & $67.96\pm0.98\%$ & $83.36\pm0.51\%$\\ % CNL
        MERL \cite{fei2020melr} & ResNet12 & 12M & & & $67.40\pm0.43\%$ & $83.40\pm0.28\%$\\ % MERL(Meta-L)
        Deep EMD v2 \cite{zhang2020deepemd} & ResNet10 & 12M& & \checkmark& $68.77\pm0.29\%$ & $84.13\pm0.53\%$ \\ 
        PAL \cite{ma2021partner} & ResNet12 & 12M & \checkmark& & $69.37\pm0.64\%$ & $84.40\pm0.44\%$\\ %PAL
        invariance-equivariance \cite{rizve2021exploring} & ResNet12 & 12M & \checkmark& & $67.28\pm0.80\%$ & $84.78\pm0.50\%$\\ 
        CSEI \cite{li2021learning} & ResNet12 & 12M & & \checkmark& $68.94\pm0.28 \%$ & $85.07\pm0.50\%$\\ %CSEI
        COSOC \cite{luo2021rectifying} & ResNet12 & 12M & & \checkmark& $69.28\pm0.49\%$ & $85.16\pm0.42\%$\\ %COSOC
        
        EASY (ours) & 2$\times$ResNet12($\frac{1}{\sqrt{2}}$) & 12M & \checkmark & \checkmark & $\mathbf{70.63 \pm 0.20\%}$ & $\mathbf{86.28 \pm 0.12\%}$\\
        \midrule
        
        S2M2R \cite{mangla2020charting} & WRN-28-10 & 36M & & &$64.93\pm0.18\%$ & $83.18\pm0.11\%$\\ %S2M2R
        LR + DC \cite{yang2021free} & WRN-28-10 & 36M & & \checkmark &$68.55\pm0.55\%$ & $82.88\pm0.42\%$\\ %LR + DC
        EASY (ours) & 3$\times$ResNet12 & 36M & \checkmark & \checkmark & $\mathbf{71.75 \pm0.19\%}$ & $\mathbf{87.15 \pm0.12\%}$\\
         
         
    \bottomrule
    \end{tabular}
    \label{tab:results_inductive_miniImageNet}
\end{table*}  

% TADAM: Oreshkin, MAML:Finn2017

==> tables/inductive/table_inductive_tiered.tex <==
\begin{table*}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on TieredImageNet in the inductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
         \midrule
        
        SimpleShot\cite{wang2019simpleshot} & ResNet18 & 11M& & & $69.09\pm0.22\%$ & $84.58\pm0.16\%$ \\ %simpleshots
        

        ProtoNet\cite{Snell2017} & ResNet12 & 12M & & &$65.65\pm0.92\%$ & $83.40\pm0.65\%$\\ %ProtoNet
        
        FEAT \cite{Ye2018} & ResNet12 & 12M & & &$70.80\pm 0.23 \%$& $84.79\pm 0.16\%$ \\ %FEAT
        PAL \cite{ma2021partner} & ResNet12 & 12M & \checkmark & &$72.25\pm0.72\%$ & $86.95\pm 0.47\%$\\ %PAL
        DeepEMD v2 \cite{zhang2020deepemd} & ResNet10 & 12M& & \checkmark &$74.29\pm 0.32\%$ & $86.98\pm0.60\%$ \\ 
        MERL \cite{fei2020melr} & ResNet12 & 12M & & & $72.14\pm0.51 \%$ & $87.01\pm 0.35\%$ \\ %MERL
        
        COSOC\cite{luo2021rectifying} & ResNet12 & 12M & &\checkmark & $73.57\pm0.43\%$ & $87.57\pm0.10\%$\\ %COSOC
        CNL \cite{zhao2021looking} & ResNet12 & 12M & & & $73.42 \pm 0.95\%$  &$87.72\pm 0.75\%$ \\ %CNL
        
 
        
        
        invariance-equivariance \cite{rizve2021exploring} & ResNet12 & 12M & \checkmark & & $72.21\pm 0.90\%$&$87.08\pm0.58\%$\\   
        CSEI \cite{li2021learning} & ResNet12 & 12M &  & &$73.76\pm0.32\%$ & $87.83\pm0.59\%$ \\ %CSEI
        ASY (ours) & ResNet12 & 12M &  & \checkmark & $\mathbf{74.31\pm 0.22\%}$ & $\mathbf{87.86 \pm 0.15\%}$\\

         \midrule
        S2M2R \cite{mangla2020charting} & WRN-28-10 & 36M & &&$73.71\pm 0.22\%$ & $\mathbf{88.52\pm0.14\%}$\\ %S2M2R
        EASY (ours) & 3$\times$ResNet12 & 36M & \checkmark & \checkmark & $\mathbf{74.71 \pm0.22\%}$ & $88.33 \pm 0.14\%$\\

    \bottomrule
    \end{tabular}
    \label{tab:results_inductive_tieredImageNet}
\end{table*}


==> tables/transductif/cifarfs.tex <==
\begin{table*}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on CIFAR-FS in the transductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
         \midrule
        SSR \cite{Shen} & ResNet12& 12M & & & $76.80\pm0.60\%$  & $83.70\pm0.40\% $ \\
        iLPC\cite{Lazarou} & ResNet12& 12M & & \checkmark& $77.14\pm 0.95\%$ &$85.23\pm0.55\%$ \\
        DPGN \cite{Yang_2020_CVPR} & ResNet12& 12M & & & $77.90\pm0.50\%$  & $90.02\pm0.40\% $ \\
        ECKPN \cite{Chen2021} & ResNet12& 12M & & & $79.20\pm0.40\%$  & $\mathbf{91.00\pm0.50\%} $ \\
        EASY (ours) & 2$\times$ResNet12($\frac{1}{\sqrt{2}}$) & 12M & \checkmark & \checkmark & $\mathbf{83.56 \pm 0.23\%}$ & $89.64 \pm 0.15\%$\\
         \midrule
        SSR \cite{Shen} & WRN-28-10& 36M & & & $81.60\pm0.60\%$  & $86.00\pm0.40\% $ \\
        Transductive fine-tuning (train+val) \cite{Dhillon2019} & WRN-28-10& 36M & &  &$78.36\pm0.70\%$ & $87.54\pm0.49\%$\\
        iLPC\cite{Lazarou} & WRN-28-10& 36M & & \checkmark& $86.51\pm 0.75\%$ &$90.60\pm0.48\%$ \\
        PT+MAP\cite{Hu2021} & WRN-28-10& 36M & & & $\mathbf{87.69\pm 0.23\%}$ &$\mathbf{90.68\pm0.15\%}$ \\
        EASY (ours) & 3$\times$ResNet12 & 36M & \checkmark & \checkmark & $84.60\pm 0.22\%$ & $90.12 \pm 0.15\%$\\
        
    \bottomrule
    \end{tabular}
    \label{tab:results_transductive_FC100}
\end{table*}





==> tables/transductif/cubfs.tex <==
\begin{table*}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on CUB-FS in the transductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
         \midrule
        TIM-GD \cite{boudiaf2020transductive} & ResNet18 & 11M & &  &$82.20\quad\quad\quad\%$ & $90.80\quad\quad\quad\%$\\ 
        ODC \cite{Qi2021} & ResNet18 & 11M & &  &$85.87\quad\quad\quad\%$ & $94.97\quad\quad\quad\%$\\
        
        DPGN \cite{Yang_2020_CVPR} & ResNet12& 12M & & & $75.71\pm0.47\%$  & $91.48\pm0.33\% $ \\
        ECKPN \cite{Chen2021} & ResNet12& 12M & & & $77.43\pm0.54\%$  & $92.21\pm0.41\% $ \\
        iLPC\cite{Lazarou} & ResNet12& 12M & & \checkmark & $89.00\pm 0.70\%$ &$92.74\pm0.35\%$ \\
        Rot+KD+POODLE\cite{Le2021} & ResNet12 & 12M & \checkmark & & $\mathbf{89.93\quad\quad\quad\%}$ &$\mathbf{93.78\quad\quad\quad\%}$ \\
        EASY (ours) & 4$\times$ResNet12($\frac{1}{2}$) & 12M & \checkmark & \checkmark & $87.53 \pm 0.21\%$ & $92.92 \pm 0.10\%$\\

        \midrule
        LR+DC \cite{yang2021free} & WRN-28-10& 36M & & & $ 79.56\pm0.87\%$  & $90.67\pm0.35\% $ \\
        PT+MAP\cite{Hu2021} & WRN-28-10& 36M & & & $\mathbf{91.55\pm 0.19\%}$ &$93.99\pm0.10\%$ \\
        iLPC\cite{Lazarou} & WRN-28-10& 36M & & \checkmark & $91.03\pm 0.63\%$ &$\mathbf{94.11\pm0.30\%}$ \\
        EASY (ours) & 3$\times$ResNet12 & 36M & \checkmark & \checkmark & $87.67 \pm 0.21\%$ & $93.30 \pm 0.09\%$\\

    \bottomrule
    \end{tabular}
    \label{tab:results_transductive_cubfs}
\end{table*}



==> tables/transductif/fc100.tex <==
\begin{table*}[!ht]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on FC-100 in the transductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
         \midrule

        
         EASY (ours) & 2$\times$ResNet12($\frac{1}{\sqrt{2}}$) & 12M & \checkmark & \checkmark & $\mathbf{52.19 \pm 0.25\%}$ & $\mathbf{65.74\pm 0.20\%}$\\
         \midrule
        SIB+E$^3$BM \cite{Liu2020} & WRN-28-10 & 36M & & & $46.00\quad\quad\quad\%$ & $57.10\quad\quad\quad\%$\\
        Transductive fine-tuning (train) \cite{Dhillon2019} & WRN-28-10& 36M & &  &$43.16\pm0.59\%$ & $57.57\pm0.55\%$\\
        ODC \cite{Qi2021}    & WRN-28-10& 36M & &  &$47.18\pm0.30\%$ & $59.21\pm0.56\%$\\ 
        Transductive fine-tuning (train+val) \cite{Dhillon2019} & WRN-28-10& 36M & &  &$50.44\pm0.68\%$ & $65.74\pm0.60\%$\\

        EASY (ours) & 3$\times$ResNet12 & 36M & \checkmark & \checkmark & $\mathbf{52.18 \pm 0.25\%}$& $\mathbf{66.35 \pm 0.20\%}$\\

    \bottomrule
    \end{tabular}
    \label{tab:results_transductive_FC100}
\end{table*}


==> tables/transductif/miniimagenet.tex <==
\begin{table*}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on miniImageNet in the transductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
        \midrule
        TIM-GD \cite{boudiaf2020transductive} & ResNet18 & 11M & &  &$73.90\quad\quad\quad\%$ & $85.00\quad\quad\quad\%$\\ 
        ODC \cite{Qi2021} & ResNet18 & 11M & &  &$77.20\pm0.36\%$ & $87.11\pm0.42\%$\\ 
        PEM$_n$E-BMS$^*$  \cite{hu2021squeezing} & ResNet18 & 11M & &  &$\mathbf{80.56\pm0.27\%}$ & $\mathbf{87.98\pm0.14\%}$\\
        SSR \cite{Shen} & ResNet12& 12M & & & $ 68.10\pm0.60\%$  & $76.90\pm0.40\% $ \\
        iLPC\cite{Lazarou} & ResNet12 & 12M & & \checkmark& $69.79\pm 0.99\%$ &$79.82\pm0.55\%$ \\
        
        EPNet\cite{rodriguez2020embedding} & ResNet12 & 12M & & & $66.50\pm 0.89\%$ &$81.60\pm0.60\%$ \\
        DPGN \cite{Yang_2020_CVPR} & ResNet12& 12M & & & $67.77\pm0.32\%$  & $84.60\pm0.43\% $ \\
        ECKPN \cite{Chen2021} & ResNet12& 12M & & & $70.48\pm0.38\%$  & $85.42\pm0.46\% $ \\
        Rot+KD+POODLE\cite{Le2021} & ResNet12 & 12M & \checkmark & & $77.56\quad\quad\quad\%$ &$85.81\quad\quad\quad\%$ \\
        EASY (ours) & 2$\times$ResNet12($\frac{1}{\sqrt{2}}$) & 12M &  \checkmark & \checkmark & $78.46 \pm 0.24\%$& $87.95 \pm 0.12\%$\\
        
         \midrule
        SSR \cite{Shen} & WRN-28-10& 36M & & & $ 72.40\pm0.60\%$  & $80.20\pm0.40\% $ \\
        Transductive fine-tuning (train+val) \cite{Dhillon2019} & WRN-28-10& 36M & &  &$68.11\pm0.69\%$ & $80.36\pm0.50\%$\\ 
        SIB+E$^3$BM \cite{Liu2020} & WRN-28-10 & 36M & & & $71.40\quad\quad\quad\%$ & $81.20\quad\quad\quad\%$\\ 
        LR+DC \cite{yang2021free} & WRN-28-10& 36M & & & $ 68.57\pm0.55\%$  & $82.88\pm0.42\% $ \\
        EPNet\cite{rodriguez2020embedding} &  WRN-28-10 & 36M  & & & $70.74\pm 0.85\%$ &$84.34\pm0.53\%$ \\
        TIM-GD \cite{boudiaf2020transductive} & WRN-28-10& 36M & &  &$77.80\quad\quad\quad\%$ & $87.40\quad\quad\quad\%$\\ 
        PT+MAP\cite{Hu2021}  & WRN-28-10& 36M & &  & $82.92\pm 0.26\%$ &$88.82\pm0.13\%$ \\
        iLPC\cite{Lazarou}   & WRN-28-10& 36M & & \checkmark& $83.05\pm 0.79\%$ &$88.82\pm0.42\%$ \\
        ODC \cite{Qi2021}    & WRN-28-10& 36M & &  &$80.64\pm0.34\%$ & $89.39\pm0.39\%$\\ 
        
        PEM$_n$E-BMS$^*$ \cite{hu2021squeezing} & WRN-28-10 & 36M & & &$\mathbf{83.35\pm0.25\%}$ & $\mathbf{89.53\pm0.13\%}$\\ 
        EASY (ours) & 3$\times$ResNet12 & 36M & \checkmark & \checkmark & $79.44 \pm 0.24\%$& $88.43 \pm 0.12\%$\\
    \bottomrule
    \end{tabular}
    \label{tab:results_transductive_miniImageNet}
\end{table*}


==> tables/transductif/table_inductive_CIFARFS.tex <==
\begin{table*}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on CIFAR-FS in the inductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
         \midrule
         S2M2R \cite{mangla2020charting} &ResNet18 &11M & \checkmark & & $63.66\pm 0.17\%$ & $76.07 \pm 0.19\%$ \\ % S2M2R
         
          R2-D2 (+ens) \cite{liu2020task} &ResNet12 &12M & \checkmark & \checkmark & $76.51\pm 0.47\%$ & $87.63 \pm 0.34\%$ \\ % R2-D2 (+ens) (+val)
         invariance-equivariance\cite{rizve2021exploring} & ResNet12 & 12M & \checkmark& & $\mathbf{77.87\pm0.85\%}$ & $\mathbf{89.74 \pm 0.57\%}$\\ %equivariance invariance
          EASY (ours) & 2$\times$ResNet12($\frac{1}{\sqrt{2}}$) & 12M & \checkmark & \checkmark & $75.24 \pm 0.20\%$ & $88.38 \pm 0.14\%$\\
       \midrule
 
        S2M2R \cite{mangla2020charting} & WRN-28-10 & 36M & & &$74.81\pm0.19\%$ & $87.47\pm0.13\%$\\ %S2M2R
         EASY (ours) & 3$\times$ResNet12 & 36M & \checkmark & \checkmark & $\mathbf{76.20\pm 0.20\%}$ & $\mathbf{89.00 \pm 0.14\%}$\\
         
    \bottomrule
    \end{tabular}
    \label{tab:results_inductive_CIFARFS}
\end{table*}


 % xu2020attentional 75.4 ± 0.2 86.8 ± 0.2
 
 % tian2020rethinking 73.9 ± 0.8 86.9 ± 0.5

==> tables/transductif/table_inductive_CUBFS.tex <==
\begin{table*}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on CUB-FS in the inductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
         \midrule
        FEAT \cite{Ye2018} & ConvNet & 0.1M & & & $68.87 \pm 0.22\%$ & $82.90\pm0.10\%$\\ % FEAT %113K parameters for conv4
         LaplacianShot \cite{MasudZiko2020} &ResNet18 &11M & & & $\mathbf{80.96\quad\quad\quad\%}$ & $88.68\quad\quad\quad\%$ \\ % Protonet

         ProtoNet \cite{Snell2017} &ResNet18 &11M & & & $66.09\pm0.92\%$ & $82.50\pm 0.58\%$ \\ % Protonet
          DeepEMD v2 \cite{zhang2020deepemd} &ResNet12 &12M &  & \checkmark & $79.27\pm 0.29\%$ & $89.80\pm 0.51\%$ \\ % DeepEMD
          EASY (ours) & 4$\times$ResNet12($\frac{1}{2}$) & 12M & \checkmark & \checkmark & $77.97 \pm 0.20\%$  & $\mathbf{91.59 \pm 0.10\%}$\\
       \midrule
 
        S2M2R \cite{mangla2020charting} & WRN-28-10 & 36M & & &$\mathbf{80.68\pm0.81\%}$ & $90.85\pm0.44\%$\\ %S2M2R
         EASY (ours) & 3$\times$ResNet12 & 36M & \checkmark & \checkmark & $78.56 \pm 0.19\%$ & $\mathbf{91.93 \pm 0.10\%}$\\
         
    \bottomrule
    \end{tabular}
    \label{tab:results_inductive_CUBFS}
\end{table*}



==> tables/transductif/table_inductive_FC-100.tex <==
\begin{table*}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on FC-100 in the inductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
         \midrule
        DeepEMD v2\cite{zhang2020deepemd} & ResNet10 & 12M & & \checkmark&$46.60\pm0.26\%  $&$ 63.22 \pm 0.71\%$ \\ 
        TADAM\cite{Oreshkin} &ResNet12 & 12M & & & $40.10 \pm 0.40\%$ & $56.10\pm 0.40\%$ \\
        ProtoNet\cite{Snell2017} &ResNet12 & 12M & & & $41.54 \pm 0.76\%$ & $57.08\pm 0.76\%$ \\ %ProtoNet
        invariance-equivariance \cite{rizve2021exploring} & ResNet12 & 12M& \checkmark& & $47.76  \pm 0.77\%$ & $\mathbf{65.30 \pm 0.76 \%}$\\ %equivariance invariance
        R2-D2 (+ens) \cite{liu2020task} &ResNet12 & 12M & \checkmark &  \checkmark&  $44.75\pm 0.43\%$ & $59.94\pm0.41 \%$ \\ 
        EASY (ours) & 2$\times$ResNet12($\frac{1}{\sqrt{2}}$) & 12M & \checkmark & \checkmark & $\mathbf{47.78 \pm 0.20\%}$ & $65.24 \pm 0.19\%$\\
         
    \bottomrule
    \end{tabular}
    \label{tab:results_inductive_FC100}
\end{table*}

% 

==> tables/transductif/table_inductive_miniImageNet.tex <==
\begin{table*}[!ht]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on miniImageNet in the inductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
         \midrule
        SimpleShot \cite{wang2019simpleshot} & ResNet18 & 11M & & &$62.85\pm0.20\%$ & $80.02\pm0.14\%$\\ %SimpleShot
        Baseline++ \cite{Chen2019} & ResNet10 & 12M& & & $53.97\pm0.79\%$ & $75.90\pm0.61\%$ \\ %Baseline++
        TADAM\cite{Oreshkin} &ResNet12 & 12M & & & $58.50 \pm 0.30\%$ & $76.70\pm 0.30\%$ \\
        ProtoNet \cite{Snell2017} & ResNet12 & 12M & & &$60.37\pm0.83\%$ & $78.02\pm0.57\%$\\ %ProtoNet
        R2-D2 (+ens) (+val) \cite{liu2020task} & ResNet12 & 12M & \checkmark &  \checkmark& $65.95\pm0.45\%$ & $81.96\pm0.32\%$\\
        FEAT \cite{Ye2018} & ResNet12 & 12M & & & $66.78\quad \quad \quad\%$ & $82.05\quad  \quad \quad \%$\\ % FEAT
        CNL \cite{zhao2021looking} & ResNet12 & 12M & & & $67.96\pm0.98\%$ & $83.36\pm0.51\%$\\ % CNL
        MERL \cite{fei2020melr} & ResNet12 & 12M & & & $67.40\pm0.43\%$ & $83.40\pm0.28\%$\\ % MERL(Meta-L)
        Deep EMD v2 \cite{zhang2020deepemd} & ResNet10 & 12M& & \checkmark& $68.77\pm0.29\%$ & $84.13\pm0.53\%$ \\ 
        PAL \cite{ma2021partner} & ResNet12 & 12M & \checkmark& & $69.37\pm0.64\%$ & $84.40\pm0.44\%$\\ %PAL
        invariance-equivariance \cite{rizve2021exploring} & ResNet12 & 12M & \checkmark& & $67.28\pm0.80\%$ & $84.78\pm0.50\%$\\ 
        CSEI \cite{li2021learning} & ResNet12 & 12M & & \checkmark& $68.94\pm0.28 \%$ & $85.07\pm0.50\%$\\ %CSEI
        COSOC \cite{luo2021rectifying} & ResNet12 & 12M & & \checkmark& $69.28\pm0.49\%$ & $85.16\pm0.42\%$\\ %COSOC
        
        EASY (ours) & 2$\times$ResNet12($\frac{1}{\sqrt{2}}$) & 12M & \checkmark & \checkmark & $\mathbf{70.63 \pm 0.20\%}$ & $\mathbf{86.28 \pm 0.12\%}$\\
        \midrule
        
        S2M2R \cite{mangla2020charting} & WRN-28-10 & 36M & & &$64.93\pm0.18\%$ & $83.18\pm0.11\%$\\ %S2M2R
        LR + DC \cite{yang2021free} & WRN-28-10 & 36M & & \checkmark &$68.55\pm0.55\%$ & $82.88\pm0.42\%$\\ %LR + DC
        EASY (ours) & 3$\times$ResNet12 & 36M & \checkmark & \checkmark & $\mathbf{71.75 \pm0.19\%}$ & $\mathbf{87.15 \pm0.12\%}$\\
         
         
    \bottomrule
    \end{tabular}
    \label{tab:results_inductive_miniImageNet}
\end{table*}  

% TADAM: Oreshkin, MAML:Finn2017

==> tables/transductif/table_inductive_tiered.tex <==
\begin{table*}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on TieredImageNet in the inductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
         \midrule
        
        SimpleShot\cite{wang2019simpleshot} & ResNet18 & 11M& & & $69.09\pm0.22\%$ & $84.58\pm0.16\%$ \\ %simpleshots
        

        ProtoNet\cite{Snell2017} & ResNet12 & 12M & & &$65.65\pm0.92\%$ & $83.40\pm0.65\%$\\ %ProtoNet
        
        FEAT \cite{Ye2018} & ResNet12 & 12M & & &$70.80\pm 0.23 \%$& $84.79\pm 0.16\%$ \\ %FEAT
        PAL \cite{ma2021partner} & ResNet12 & 12M & \checkmark & &$72.25\pm0.72\%$ & $86.95\pm 0.47\%$\\ %PAL
        DeepEMD v2 \cite{zhang2020deepemd} & ResNet10 & 12M& & \checkmark &$74.29\pm 0.32\%$ & $86.98\pm0.60\%$ \\ 
        MERL \cite{fei2020melr} & ResNet12 & 12M & & & $72.14\pm0.51 \%$ & $87.01\pm 0.35\%$ \\ %MERL
        
        COSOC\cite{luo2021rectifying} & ResNet12 & 12M & &\checkmark & $73.57\pm0.43\%$ & $87.57\pm0.10\%$\\ %COSOC
        CNL \cite{zhao2021looking} & ResNet12 & 12M & & & $73.42 \pm 0.95\%$  &$87.72\pm 0.75\%$ \\ %CNL
        
 
        
        
        invariance-equivariance \cite{rizve2021exploring} & ResNet12 & 12M & \checkmark & & $72.21\pm 0.90\%$&$87.08\pm0.58\%$\\   
        CSEI \cite{li2021learning} & ResNet12 & 12M &  & &$73.76\pm0.32\%$ & $87.83\pm0.59\%$ \\ %CSEI
        ASY (ours) & ResNet12 & 12M &  & \checkmark & $\mathbf{74.31\pm 0.22\%}$ & $\mathbf{87.86 \pm 0.15\%}$\\

         \midrule
        S2M2R \cite{mangla2020charting} & WRN-28-10 & 36M & &&$73.71\pm 0.22\%$ & $\mathbf{88.52\pm0.14\%}$\\ %S2M2R
        EASY (ours) & 3$\times$ResNet12 & 36M & \checkmark & \checkmark & $\mathbf{74.71 \pm0.22\%}$ & $88.33 \pm 0.14\%$\\

    \bottomrule
    \end{tabular}
    \label{tab:results_inductive_tieredImageNet}
\end{table*}


==> tables/transductif/tiered.tex <==
\begin{table*}[!ht]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods in the literature on TieredImageNet in the transductive setting, compared with the proposed solution.}
    \centering
    \small
    \begin{tabular}{lcccccc}
    \toprule
         Method & Backbone & Params & E/D & AS & 1-shot & 5-shot \\
        \midrule
        PT+MAP\cite{Hu2021} & DenseNet121& 8M & & & $85.67\pm 0.26\%$ &$90.45\pm0.14\%$ \\
        
        TIM-GD \cite{boudiaf2020transductive} & ResNet18 & 11M & &  &$79.90\quad\quad\quad\%$ & $88.50\quad\quad\quad\%$\\ 
        ODC \cite{Qi2021} & ResNet18 & 11M & &  &$\mathbf{83.73\pm0.36\%}$ & $\mathbf{90.46\pm0.46\%}$\\ 
        
        SSR \cite{Shen} & ResNet12& 12M & & & $81.20\pm0.60\%$  & $85.70\pm0.40\% $ \\
        Rot+KD+POODLE\cite{Le2021} & ResNet12 & 12M & \checkmark & & $79.67\quad\quad\quad\%$ &$86.96\quad\quad\quad\%$ \\
        DPGN \cite{Yang_2020_CVPR} & ResNet12& 12M & & & $72.45\pm0.51\%$  & $87.24\pm0.39\% $ \\
        EPNet\cite{rodriguez2020embedding} & ResNet12 & 12M & & & $76.53\pm 0.87\%$ &$87.32\pm0.64\%$ \\
        ECKPN \cite{Chen2021} & ResNet12& 12M & & & $73.59\pm0.45\%$  & $88.13\pm0.28\% $ \\
        iLPC\cite{Lazarou} & ResNet12& 12M & & \checkmark& $83.49\pm 0.88\%$ &$89.48\pm0.47\%$ \\
        ASY (ours) & ResNet12 & 12M &  & \checkmark & $80.75\pm 0.27\%$ & $88.86 \pm 0.14\%$\\
        
        \midrule
        SIB+E$^3$BM \cite{Liu2020} & WRN-28-10 & 36M & & & $75.60\quad\quad\quad\%$ & $84.30\quad\quad\quad\%$\\
        SSR \cite{Shen} & WRN-28-10& 36M & & & $79.50\pm0.60\%$  & $84.80\pm0.40\% $ \\
        Transductive fine-tuning (train+val) \cite{Dhillon2019} & WRN-28-10& 36M & &  &$72.87\pm0.71\%$ & $86.15\pm0.50\%$\\ 
        TIM-GD \cite{boudiaf2020transductive} & WRN-28-10& 36M & &  &$82.10\quad\quad\quad\%$ & $89.80\quad\quad\quad\%$\\ 
        LR+DC \cite{yang2021free} & WRN-28-10& 36M & & & $ 78.19\pm0.25\%$  & $89.90\pm0.41\% $ \\ %LR+DC (trasductif)
        EPNet\cite{rodriguez2020embedding} & WRN-28-10 & 36M & & & $78.50\pm 0.91\%$ &$88.36\pm0.57\%$ \\
        ODC \cite{Qi2021} &  WRN-28-10& 36M & &  &$85.22\pm0.34\%$ & $91.35\pm0.42\%$\\ 
        iLPC\cite{Lazarou} & WRN-28-10& 36M & & \checkmark& $\mathbf{88.50\pm 0.75\%}$ &$\mathbf{92.46\pm0.42\%}$ \\
        PEM$_n$E-BMS$^*$ \cite{hu2021squeezing} & WRN-28-10 & 36M & & &$86.07\pm0.25\%$ & $91.09\pm0.14\%$\\
        EASY (ours) & 3$\times$ResNet12 & 36M & \checkmark & \checkmark & $81.01 \pm 0.27\%$ & $89.29 \pm 0.14\%$\\

    \bottomrule
    \end{tabular}
    \label{tab:results_transductive_tieredImageNet}
\end{table*}


==> tables2/transductive_yuqingresults/cifarfs.tex <==
\begin{table}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods and proposed solution on \textbf{CIFAR-FS} in \textbf{transductive} setting.}
    \centering
    \begin{tabular}{p{0.2cm}p{3.7cm}>{\centering\arraybackslash}p{1.6cm}>{\centering\arraybackslash}p{1.6cm}}
    \toprule
         & Method& 1-shot & 5-shot \\
         \midrule
        \multirow{5}{*}{\rotatebox[origin=c]{90}{$\leq 12M$}
        $\left\{\vphantom{\begin{tabular}{c}~\\~\\~\\~\\~\\\end{tabular}}\right.$}
        &SSR~\cite{Shen} & $76.80\pm0.60$  & $83.70\pm0.40 $ \\
        &iLPC~\cite{Lazarou}& $77.14\pm 0.95$ &$85.23\pm0.55$ \\
        &DPGN~\cite{Yang_2020_CVPR} & $77.90\pm0.50$  & $90.02\pm0.40 $ \\
        &ECKPN~\cite{Chen2021} & $79.20\pm0.40$  & $\mathbf{91.00\pm0.50} $ \\
        %&EASY 2$\times$ResNet12($\frac{1}{\sqrt{2}}$)^* & $\mathbf{83.56 \pm 0.23}$ & $89.64 \pm 0.15$\\
        &EASY 2$\times$ResNet12$\left(\frac{1}{\sqrt{2}}\right)$ \scriptsize{(ours)} & $\mathbf{86.40 \pm 0.23}$ & $89.75 \pm 0.15$\\
         \midrule
        \multirow{5}{*}{\rotatebox[origin=c]{90}{$36M$}
        $\left\{\vphantom{\begin{tabular}{c}~\\~\\~\\~\\~\\\end{tabular}}\right.$}
        &SSR~\cite{Shen} & $81.60\pm0.60$  & $86.00\pm0.40 $ \\
        &fine-tuning (train+val)~\cite{Dhillon2019} &$78.36\pm0.70$ & $87.54\pm0.49$\\
        &iLPC~\cite{Lazarou}& $86.51\pm 0.75$ &$90.60\pm0.48$ \\
        &PT+MAP~\cite{Hu2021}& $\mathbf{87.69\pm 0.23}$ &$\mathbf{90.68\pm0.15}$ \\
        %&EASY 3$\times$ResNet12^* & $84.60\pm 0.22$ & $90.12 \pm 0.15$\\
        &EASY 3$\times$ResNet12 \scriptsize{(ours)} & $86.96\pm 0.22$ & $90.30 \pm 0.15$\\
        
    \bottomrule
    \end{tabular}
    \label{tab:results_transductive_FC100}
\end{table}





==> tables2/transductive_yuqingresults/cubfs.tex <==
\begin{table}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods and proposed solution on \textbf{CUB-FS} in \textbf{transductive} setting.}
    \centering
    \begin{tabular}{p{0.2cm}p{3.7cm}>{\centering\arraybackslash}p{1.6cm}>{\centering\arraybackslash}p{1.6cm}}
    \toprule
         & Method& 1-shot & 5-shot \\
         \midrule
        \multirow{7}{*}{\rotatebox[origin=c]{90}{$\leq 12M$}
        $\left\{\vphantom{\begin{tabular}{c}~\\~\\~\\~\\~\\~\\~\\\end{tabular}}\right.$}
        & TIM-GD~\cite{boudiaf2020transductive} &$82.20\quad\quad\quad$ & $90.80\quad\quad\quad$\\ 
        & ODC~\cite{Qi2021} &$85.87\quad\quad\quad$ & $94.97\quad\quad\quad$\\
        
        & DPGN~\cite{Yang_2020_CVPR} & $75.71\pm0.47$  & $91.48\pm0.33 $ \\
        & ECKPN~\cite{Chen2021} & $77.43\pm0.54$  & $92.21\pm0.41 $ \\
        & iLPC~\cite{Lazarou} & $89.00\pm 0.70$ &$92.74\pm0.35$ \\
        & Rot+KD+POODLE~\cite{Le2021} & $89.93\quad\quad\quad$ &$\mathbf{93.78\quad\quad\quad}$ \\
        %& EASY 4$\times$ResNet12($\frac{1}{2}$)^* & $87.53 \pm 0.21$ & $92.92 \pm 0.10$\\
        & EASY 4$\times$ResNet12$\left(\frac{1}{2}\right)$ \scriptsize{(ours)} & $\mathbf{90.41 \pm 0.19}$ & $93.58 \pm 0.10$\\

        \midrule
        \multirow{4}{*}{\rotatebox[origin=c]{90}{$36M$}
        $\left\{\vphantom{\begin{tabular}{c}~\\~\\~\\~\\\end{tabular}}\right.$}
        & LR+DC~\cite{yang2021free} & $ 79.56\pm0.87$  & $90.67\pm0.35 $ \\
        & PT+MAP~\cite{Hu2021} & $\mathbf{91.55\pm 0.19}$ &$93.99\pm0.10$ \\
        & iLPC~\cite{Lazarou} & $91.03\pm 0.63$ &$\mathbf{94.11\pm0.30}$ \\
        %& EASY 3$\times$ResNet12^* & $87.67 \pm 0.21$ & $93.30 \pm 0.09$\\
        & EASY 3$\times$ResNet12 \scriptsize{(ours)} & $90.76 \pm 0.19$ & $93.90 \pm 0.09$\\

    \bottomrule
    \end{tabular}
    \label{tab:results_transductive_cubfs}
\end{table}



==> tables2/transductive_yuqingresults/fc100.tex <==
\begin{table}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methodsand proposed solution on \textbf{FC-100} in \textbf{transductive} setting.}
    \centering
    \begin{tabular}{p{0.2cm}p{3.7cm}>{\centering\arraybackslash}p{1.6cm}>{\centering\arraybackslash}p{1.6cm}}
    \toprule
         & Method& 1-shot & 5-shot \\
         \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{$\leq 12M$}
        $\left\{\vphantom{\begin{tabular}{c}~\\~\\~\\\end{tabular}}\right.$}
        &&&\\
        
         %\begin{turn}{90}\hspace{-0.2cm} \scriptsize{$12M$}\end{turn}&EASY 2$\times$ResNet12($\frac{1}{\sqrt{2}}$)^* & $\mathbf{52.19 \pm 0.25}$ & $\mathbf{65.74\pm 0.20}$\\
         &EASY 2$\times$ResNet12$\left(\frac{1}{\sqrt{2}}\right)$ \scriptsize{(ours)} & $\mathbf{54.68 \pm 0.25}$ & $\mathbf{66.19\pm 0.20}$\\
         &&&\\
         \midrule
        \multirow{5}{*}{\rotatebox[origin=c]{90}{$36M$}
        $\left\{\vphantom{\begin{tabular}{c}~\\~\\~\\~\\~\\\end{tabular}}\right.$}
        &SIB+E$^3$BM~\cite{Liu2020} & $46.00\quad\quad\quad$ & $57.10\quad\quad\quad$\\
        &fine-tuning (train)~\cite{Dhillon2019}  &$43.16\pm0.59$ & $57.57\pm0.55$\\
        &ODC~\cite{Qi2021} &$47.18\pm0.30$ & $59.21\pm0.56$\\ 
        &fine-tuning (train+val)~\cite{Dhillon2019} &$50.44\pm0.68$ & $65.74\pm0.60$\\

        %&EASY 3$\times$ResNet12^* & $\mathbf{52.18 \pm 0.25}$& $\mathbf{66.35 \pm 0.20}$\\
        &EASY 3$\times$ResNet12 \scriptsize{(ours)} & $\mathbf{55.11 \pm 0.25}$& $\mathbf{67.09 \pm 0.20}$\\

    \bottomrule
    \end{tabular}
    \label{tab:results_transductive_FC100}
\end{table}


==> tables2/transductive_yuqingresults/miniimagenet.tex <==
\begin{table}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods and proposed solution on \textbf{MiniImageNet} in \textbf{transductive} setting.}
    \centering
    \begin{tabular}{p{0.2cm}p{3.7cm}>{\centering\arraybackslash}p{1.6cm}>{\centering\arraybackslash}p{1.6cm}}
    \toprule
         & Method& 1-shot & 5-shot \\
         \midrule
        \multirow{10}{*}{\rotatebox[origin=c]{90}{$\leq 12M$}
        $\left\{\vphantom{\begin{tabular}{c}~\\~\\~\\~\\~\\~\\~\\~\\~\\~\\\end{tabular}}\right.$}
        & TIM-GD~\cite{boudiaf2020transductive} &$73.90\quad\quad\quad$ & $85.00\quad\quad\quad$\\ 
        & ODC~\cite{Qi2021} &$77.20\pm0.36$ & $87.11\pm0.42$\\ 
        & PEM$_n$E-BMS$^*$ ~\cite{hu2021squeezing}  &$80.56\pm0.27$ & $87.98\pm0.14$\\
        & SSR~\cite{Shen} & $ 68.10\pm0.60$  & $76.90\pm0.40 $ \\
        & iLPC~\cite{Lazarou} & $69.79\pm 0.99$ &$79.82\pm0.55$ \\
        
        & EPNet~\cite{rodriguez2020embedding}& $66.50\pm 0.89$ &$81.60\pm0.60$ \\
        & DPGN~\cite{Yang_2020_CVPR} & $67.77\pm0.32$  & $84.60\pm0.43 $ \\
        & ECKPN~\cite{Chen2021} & $70.48\pm0.38$  & $85.42\pm0.46 $ \\
        & Rot+KD+POODLE~\cite{Le2021} & $77.56\quad\quad\quad$ &$85.81\quad\quad\quad$ \\
        %& EASY 2$\times$ResNet12($\frac{1}{\sqrt{2}}$)^*  & $78.46 \pm 0.24$& $87.95 \pm 0.12$\\
        & EASY 2$\times$ResNet12$\left(\frac{1}{\sqrt{2}}\right)$ \scriptsize{(ours)}  & $\mathbf{82.18 \pm 0.24}$& $\mathbf{88.57 \pm 0.12}$\\
        
         \midrule
         \multirow{11}{*}{\rotatebox[origin=c]{90}{$36M$}
        $\left\{\vphantom{\begin{tabular}{c}~\\~\\~\\~\\~\\~\\~\\~\\~\\~\\~\\\end{tabular}}\right.$}
        & SSR~\cite{Shen} & $ 72.40\pm0.60$  & $80.20\pm0.40 $ \\
        & fine-tuning(train+val)~\cite{Dhillon2019} &$68.11\pm0.69$ & $80.36\pm0.50$\\ 
        & SIB+E$^3$BM~\cite{Liu2020} & $71.40\quad\quad\quad$ & $81.20\quad\quad\quad$\\ 
        & LR+DC~\cite{yang2021free} & $ 68.57\pm0.55$  & $82.88\pm0.42 $ \\
        & EPNet~\cite{rodriguez2020embedding} & $70.74\pm 0.85$ &$84.34\pm0.53$ \\
        & TIM-GD~\cite{boudiaf2020transductive}  &$77.80\quad\quad\quad$ & $87.40\quad\quad\quad$\\ 
        & PT+MAP~\cite{Hu2021}  & $82.92\pm 0.26$ &$88.82\pm0.13$ \\
        & iLPC~\cite{Lazarou}   & $83.05\pm 0.79$ &$88.82\pm0.42$ \\
        & ODC~\cite{Qi2021}    &$80.64\pm0.34$ & $89.39\pm0.39$\\ 
        
        & PEM$_n$E-BMS$^*$~\cite{hu2021squeezing}  &$\mathbf{83.35\pm0.25}$ & $\mathbf{89.53\pm0.13}$\\ 
        %& EASY 3$\times$ResNet12^{*}  & $79.44 \pm 0.24$& $88.43 \pm 0.12$\\
        & EASY 3$\times$ResNet12 \scriptsize{(ours)}  & $83.31 \pm 0.24$& $89.22 \pm 0.12$\\
    \bottomrule
    \end{tabular}
    \label{tab:results_transductive_miniImageNet}
\end{table}


==> tables2/transductive_yuqingresults/tiered.tex <==
\begin{table}[!htbp]
    \caption{1-shot and 5-shot accuracy of state-of-the-art methods and proposed solution on \textbf{TieredImageNet} in \textbf{transductive} setting.}
    \centering
    \begin{tabular}{p{0.2cm}p{3.7cm}>{\centering\arraybackslash}p{1.6cm}>{\centering\arraybackslash}p{1.6cm}}
    \toprule
         & Method& 1-shot & 5-shot \\
         \midrule
        \multirow{10}{*}{\rotatebox[origin=c]{90}{$\leq 12M$}
        $\left\{\vphantom{\begin{tabular}{c}~\\~\\~\\~\\~\\~\\~\\~\\~\\~\\\end{tabular}}\right.$}
        & PT+MAP~\cite{Hu2021} &$85.67\pm 0.26$ &$90.45\pm0.14$ \\
        
        & TIM-GD~\cite{boudiaf2020transductive} &$79.90\quad\quad\quad$ & $88.50\quad\quad\quad$\\ 
        & ODC~\cite{Qi2021}  &$\mathbf{83.73\pm0.36}$ & $\mathbf{90.46\pm0.46}$\\ 
        
        & SSR~\cite{Shen} & $81.20\pm0.60$  & $85.70\pm0.40 $ \\
        & Rot+KD+POODLE~\cite{Le2021} & $79.67\quad\quad\quad$ &$86.96\quad\quad\quad$ \\
        & DPGN~\cite{Yang_2020_CVPR} & $72.45\pm0.51$  & $87.24\pm0.39 $ \\
        & EPNet~\cite{rodriguez2020embedding} & $76.53\pm 0.87$ &$87.32\pm0.64$ \\
        & ECKPN~\cite{Chen2021} & $73.59\pm0.45$  & $88.13\pm0.28 $ \\
        & iLPC~\cite{Lazarou} & $83.49\pm 0.88$ &$89.48\pm0.47$ \\
        %& ASY ResNet12^* & $80.75\pm 0.27$ & $88.86 \pm 0.14$\\
        & ASY ResNet12 \scriptsize{(ours)} & $82.66\pm 0.27$ & $88.60 \pm 0.14$\\
        
        \midrule
        \multirow{10}{*}{\rotatebox[origin=c]{90}{$36M$}
        $\left\{\vphantom{\begin{tabular}{c}~\\~\\~\\~\\~\\~\\~\\~\\~\\~\\\end{tabular}}\right.$}
        & SIB+E$^3$BM~\cite{Liu2020} & $75.60\quad\quad\quad$ & $84.30\quad\quad\quad$\\
        & SSR~\cite{Shen} & $79.50\pm0.60$  & $84.80\pm0.40 $ \\
        & fine-tuning (train+val)~\cite{Dhillon2019}  &$72.87\pm0.71$ & $86.15\pm0.50$\\ 
        & TIM-GD~\cite{boudiaf2020transductive}  &$82.10\quad\quad\quad$ & $89.80\quad\quad\quad$\\ 
        & LR+DC~\cite{yang2021free} & $ 78.19\pm0.25$  & $89.90\pm0.41 $ \\ %LR+DC (trasductif)
        & EPNet~\cite{rodriguez2020embedding} & $78.50\pm 0.91$ &$88.36\pm0.57$ \\
        & ODC~\cite{Qi2021}  &$85.22\pm0.34$ & $91.35\pm0.42$\\ 
        & iLPC~\cite{Lazarou} & $\mathbf{88.50\pm 0.75}$ &$\mathbf{92.46\pm0.42}$ \\
        & PEM$_n$E-BMS$^*$~\cite{hu2021squeezing} &$86.07\pm0.25$ & $91.09\pm0.14$\\
        %& EASY 3$\times$ResNet12^*  & $81.01 \pm 0.27$ & $89.29 \pm 0.14$\\
        & EASY 3$\times$ResNet12 \scriptsize{(ours)}  & $84.48 \pm 0.27$ & $89.71 \pm 0.14$\\

    \bottomrule
    \end{tabular}
    \label{tab:results_transductive_tieredImageNet}
\end{table}

